Convexification of box-constrained polynomial optimization problems via monomial patterns

Convexification is a core technique in global polynomial optimization. Currently, there are two main approaches competing in theory and practice: the approach of nonlinear programming and the approach based on positivity certificates from real algebra. The former are comparatively cheap from a computational point of view, but typically do not provide tight relaxations with respect to bounds for the original problem. The latter are typically computationally expensive, but do provide tight relaxations. We embed both kinds of approaches into a unified framework of monomial relaxations. We develop a convexification strategy that allows to trade off the quality of the bounds against computational expenses. Computational experiments show very encouraging results.

==> acknowledgements.tex <==
The authors gratefully acknowledge the support from the Deut\-sche For\-schungs\-
ge\-mein\-schaft (DFG, German Research Foundation) - 314838170, GRK 2297
MathCoRe. The second author was partially supported by the Ministry of Economy, Science and Digitalisation of the federal state Saxony-Anhalt by means of the Landesgraduierten-Stipendium. 

==> algorithm.tex <==
%We present a cutting plane algorithm that iteratively solves \eqref{P-RLX} and suggest a method for choosing a system of patterns for relaxing \eqref{POP} to \eqref{P-RLX}.
%\subsection{Cutting Plane Algorithm}\label{cutting:plane:algorithm}
In \cref{algo:cutting} we formulate a hybrid cut\-ting plane algorithm for solving \eqref{P-RLX}.
The underlying idea is to divide $\mP$ into statically used patterns $\mP^{'}$ and dynamically used patterns $\mP^{''}$. The basic constraints $\bfv_{P} \in \mM(K)_P $ for $ P\in\mP^{'}$ are always considered in the \emph{master problem} \eqref{prob:master}, while cuts are generated by solving the \emph{slave} (or separation) \emph{problems} \eqref{SP} for more involved patterns $P\in\mP^{''}$. This way $\mP^{'}$ and $\mP^{''}$ allow to control the size and problem type of the master problem. 
%
In particular, choosing $\mP^{'}$ to contain only multilinear patterns makes \eqref{prob:master} a linear program, while the slave problems may be psd cone formulations. This allows to solve \eqref{prob:master} with the dual simplex algorithm, warmstarting after the inclusion of linear cuts generated from $P\in\mP^{''}$. Similarly, in a branch-and-bound framework cuts corresponding to patterns $P\in\mP^{''}$ could be used to augment the pattern relaxation \eqref{prob:master} until the bounds are tight enough for further branching.
\begin{algorithm}[htbp]
\textbf{Input:} $\bullet$ \ finite family of patterns $\mP=\mP^{'}\cup\mP^{''}$, where $\mP^{'}$ contains statically and $\mP^{''}$ contains dynamically used patterns \ $\bullet$ \ coefficient vector $\bff\in\R^{A_{\mP}}$\ $\bullet$ \ tolerance $\varepsilon>0$ 
%\eqref{pattern:relaxation} is computational cheap to enforce by linear constraints for $\mP^{'}$ and expensive for $\mP^{''}$

\noindent
\textbf{Output:} $\mO(\varepsilon)$-optimal and $\mO(\varepsilon)$-feasible solution $\bfv^\ast(\varepsilon)$ of \eqref{P-RLX}.
\medskip
\begin{itemize}
  \item[(0)]
  Set $i=0$. 
  \item[(1)] 
  Solve the following problem 
  \renewcommand{\arraystretch}{1.2}   
  \begin{align}\tag{MP}\label{prob:master}
    \begin{array}{cl@{\,}l@{\,}lll}
    \maximize{0}  & \langle   & \multicolumn{3}{@{}l}{\bff, \bfv \,\rangle}  \\
    \for[0]{0}    &           & \bfv          & \in\R^{A_{\mP}}\\
    \st[0]{0}     &           & \bfv_{P}      &\in \mM(K)_P & \,\fa[0]{0}\, P \in \mP^{'},\\
                  &           & \rmv_{\alpha} &\in [\xmin{\alpha}{K},\xmax{\alpha}{K}]  &\,\fa[0]{0} \alpha\in A_{\mP},\\
                  &           & \bfv          & \text{satisfies } \mathrm{Ineq}^k      &\,\fa[0]{0}\, k\in [i]
    \end{array}   
  \end{align} 
  and save the minimizer as $\bfv^{i+1}$. Set $i \leftarrow i+1$.
  \item[(2)]
  Initialize $\mathrm{Ineq}^i=\emptyset$. For each pattern $P\in\mP^{''}$ determine the corresponding distance $\delta := \dist(\mM(K)_{P},\bfv_{P})$ by solving the respective separation problem \eqref{SP}. If $\delta>\varepsilon$, add $\langle \bfc^P,\bfv\rangle \ge \delta, \bfv\in\R^{A_{\mP}}$ to the set of inequalities $\mathrm{Ineq}^i$.
  \item[(3)]
  If the set $\mathrm{Ineq}^i$ is empty return $\bfv^\ast(\varepsilon):=\bfv^i$, else go to step (1).
\end{itemize}
\caption{Hybrid Cut\-ting Plane Algorithm}\label{algo:cutting}
\end{algorithm}

We are now proving finite termination and a bound on the result of \cref{algo:cutting}.
\begin{theorem}\label{05-prop:qualitive-convergence}
  For every given $\varepsilon>0$, \cref{algo:cutting} terminates after a finite number of iterations. The output satisfies
  \begin{align}\label{05-eq:proof-convergence1}
    \bfv_{P}^*              &\in \mM(K)_P       &&  \fa[-80]{3} P\in\mP^{'}   \\
    \bfv_{P}^*(\varepsilon) &\in \Neps(\mM(K))_{P} &&  \fa[-80]{3} P\in\mP^{''} .  
  \end{align}
\end{theorem}
\begin{proof}
  Assume that \cref{algo:cutting} does not terminate after a finite number of iterations. Then it produces an infinite sequence $(\bfv^i)_{i\in\N}$ such that for all $i$ there exists a $P_i\in\mP^{''}$ with 
  \[
   \bfv_{P_i}\notin\Neps(\mM(K)_{P_i}).
  \]
  Hence, there exists a pattern $P$ and an infinite sequence $(i_k)_{ k\in\N}$ satisfying $P=P_{i_k}$ for all $k$.
  Let $F^i$ be the feasible set of \eqref{prob:master} in the $i$-th iteration. Observe that by construction  $F^{i+1}\subseteq F^i$ holds and therefore $\bfv^{i_k}\in F^0$ for all $k\in\N$. Since $F^0$ is compact there exists a converging subsequence $(\tbfv^i)_{i\in\N}$ of $(\bfv^{i_k})_{k\in\N}$. Let $\tbfv=\lim\limits_{i\rightarrow\infty}\tbfv^i$. By the choice of the sequence we have
  $
  \dist(\mM(K)_P,\tbfv^i_P)>\varepsilon.
  $
  for all $i\in\N$. Hence, for $i$ large enough, $\Vert\tbfv^i_P-\tbfv_P\Vert_1<\dist(\mM(K)_P,\tbfv^i_P)$ holds. Application of  \cref{05-lem:duality-dis-sep} to the minimizers $\bfc^i, \delta_i$ of \eqref{SP} for $\bfv=\tbfv_P^i$ yields %and the H\"older inequality yield
  \begin{align*}
    \bsprod{\bfc^i}{\tbfv_P}  & = \bsprod{\bfc^i}{\tbfv_P-\tbfv^i_P} + \bsprod{\bfc^i}{\tbfv^i_P} \\
                              & = \bsprod{\bfc^i}{\tbfv_P-\tbfv^i_P} + \delta_i - \dist(\mM(K)_P,\tbfv^i_P) \\
                              & \le \|\bfc^i\|_\infty\|\tbfv_P-\tbfv^i_P\|_1 + \delta_i - \dist(\mM(K)_P,\tbfv^i_P) \\
                            & < \dist(\mM(K)_P,\tbfv^i_P) + \delta_i - \dist(\mM(K)_P,\tbfv^i_P) = \delta_i.  
  \end{align*}
  This is a contradiction since $\tbfv\in F^i$ for all $i$. 
\end{proof}
The following theorem shows that $\rmf^*(\varepsilon):=\langle \bff,\bfv^*(\varepsilon)\rangle$ converges to the optimal value $\rmf^*$ of \eqref{P-RLX}, as $\varepsilon\rightarrow 0$, and that the convergence rate depends linearly on $\varepsilon$.
\begin{theorem}\label{05-prop:quantitative-convergence}
  There exists a constant $C(K,A_{\mP})$ depending on $K$ and $A_{\mP}$ such that for every $\varepsilon>0$ the distance between the feasible set of \eqref{P-RLX} and the output $\bfv^*(\varepsilon)$ of \cref{algo:cutting} is at most $C(K,A_{\mP})\varepsilon$. Furthermore, the optimal value $\rmf^*$ of \eqref{P-RLX} satisfies
  \[
    \langle\bff,\bfv^*(\varepsilon)\rangle \le \rmf^*\le \Vert\bff\Vert_{\infty}C(K,A_{\mP})\varepsilon + \langle\bff,\bfv^*(\varepsilon)\rangle.
  \]
\end{theorem}
For the proof we use the following lemma, which is an adaptation of \cite[Lem. 1.8.9]{schneider2014}.

\begin{lemma}\label{05-lem:dist-cap}
	Let $X, X^1,\ldots,X^m$ be nonempty compact convex subsets of $\R^A$ such that the intersection $Y:=X^1 \cap \ldots \cap X^m$ contains an $l_1$-ball of radius $\rho>0$ as a subset and the inclusion $X^i \subseteq X$ holds for every $i \in [m]$. Let $\epsilon>0$ and let $\bfx$ be a point of $X$ satisfying $\dist(X^i,\bfx) \le \epsilon$ for every $i \in [m]$. Then 
	\[
		\dist(Y, \bfx) \le \frac{\epsilon}{\rho} \diam(X).
	\]
\end{lemma}
\begin{proof}
  Since the assertion is invariant under translation, we assume that the $l_1$-ball of radius $\rho$ contained in $Y$ is centered at the origin, that is, $B:=\{\bfx\in\R^A:\|\bfx\|_1\le \rho\} \subseteq Y$.
  For each $i \in[m]$, choose a point $\bfx^i \in X^i$ with $\|\bfx-\bfx^i\|_1 \le \epsilon$. We claim that the point $\bfy:=\frac{\rho}{\rho+\epsilon} \bfx$ belongs to $Y$. For every $i \in [m]$, we fix $\bfp^i \in \R^A$ defined by the equality
  \[
    \bfy=\frac{\rho}{\rho+ \epsilon} \bfx = \frac{\epsilon}{\rho+\epsilon} \bfp^i + \frac{\rho}{\rho+\epsilon} \bfx^i.
  \]
  By construction, $\bfy$ is a convex combination of $\bfp^i$ and $\bfx^i$. Thus, for verifying the claim, it suffices to show that $\bfp^i \in B$ for every $i \in [m]$. Indeed, if $\bfp^i \in B$, then since $B$ is a subset of $X^i$ and $\bfp^i$ belongs to $X^i$, we obtain that $\bfy \in X^i$ for every $i \in [m]$, which verifies the claim. The point $\bfp^i$ can be defined explicitly as 
  \[
    \bfp^i = \frac{\rho}{\epsilon} (\bfx-\bfx^i).
  \]
  Since $\|\bfx-\bfx^i\| \le \epsilon$, we immediately get $\bfp^i \in B$. The proof is concluded by estimating the distance between $\bfx$ and $\bfy$ 
  \[
    \dist(Y,\bfx) \le \|\bfy-\bfx\|_1  = \frac{\epsilon}{\rho+\epsilon} \left\| \bfx \right\|_1.
  \] 
  Here, $\frac{\epsilon}{\rho+\epsilon}\le\frac{\epsilon}{\rho}$, while $\|\bfx\|_1$ is the $l_1$-distance between $\0$ and $\bfx$ both belonging to $X$, which implies $\|\bfx \|_1 \le \diam(X)$. Thus, we arrive at the desired estimate of $\dist(Y,\bfx)$. 
\end{proof}
\begin{proof}[Proof of \cref{05-prop:quantitative-convergence}]
  If some pattern $P\in\mP$ contains $\0$, then $\0\in A_{\mP}$ and the constraint $\rmv_\alpha\in [\xmin{\alpha}{K},\xmax{\alpha}{K}]$ with $\alpha=0$ occurring in $\mathrm{Ineq}^0$ can be formulated as the equality $\rmv_{\0}=1$. This shows that all solutions generated during the iteration satisfy the constraint $\rmv_{\0}=1$. Using this observation and \cref{05-prop:qualitive-convergence}, which yields $\bfv_{P}^*(\varepsilon)\in\Neps(\mM(K)_{P})$, we obtain $\bfv_{P\setminus\{\0\}}^*(\varepsilon)\in\Neps(\mM(K)_{P\setminus\{\0\}})$. We can therefore remove $\0$ from all patterns and assume that $\0\not\in P$ holds for every $P\in\mP$. The feasible set of \eqref{P-RLX} is the intersection of 
  \begin{align*}
    F^P &:=\{\bfv\in\R^{A_{\mP}}:\bfv_{P}\in\mM(K)_{P}\}\cap\Box(\xmin{A_{\mP}}{K},\xmax{A_{\mP}}{K})
  \end{align*}
  for all $P\in\mP$. We show that $\mM(K)_{A_{\mP}}$ is full-dimensional by assuming the contrary. Then $\mM(K)_{A_{\mP}}$ is contained in a linear subspace $\{\bfv\in\R^{A_{\mP}}:\langle\bfc,\bfv\rangle=0\}$ given by $\bfc\in\R^{A_{\mP}}$ with $\bfc\not=\0$. Hence $\langle\bfc,\m(\bfx)_{A_{\mP}}\rangle$ is a polynomial in $\bfx$ vanishing on a $n$-dimensional set $K$. This implies $\bfc=\0$, which is a contradiction. Hence, $\mM(K)_{A_{\mP}}$ is full dimensional and therefore contains a ball with radius $R(K,A_{\mP})$ depending only on $K$ and $A_{\mP}$. The feasible set $\bigcap_{P\in\mP}F^P$ of \eqref{P-RLX} contains $\mM(K)_{A_{\mP}}$ and therefore the mentioned ball. The diameter $D(K,A_{\mP})$ of $\Box(\xmin{A_{\mP}}{K},\xmax{A_{\mP}}{K})$ depends only on $K$ and $A_{\mP}$. From $\bfv^*(\varepsilon)\in\bigcap_{P\in\mP^{'}}F^P\cap\bigcap_{P\in\mP^{''}}\Neps(F^P)\cap\Box(\xmin{A_{\mP}}{K},\xmax{A_{\mP}}{K})$ and \cref{05-lem:dist-cap} it follows that 
  \[
    \dist(\bigcap\limits_{P\in\mP}(F^P\cap\Box(\xmin{A_{\mP}}{K},\xmax{A_{\mP}}{K})),\bfv^*(\varepsilon))\le\underbrace{\frac{D(K,A_{\mP})}{R(K,A_{\mP})}}_{:=C(K,A_{\mP})}\varepsilon.
  \]
  At last, let $\bfv\in\bigcap_{P\in\mP}F^P$ satisfy $\|\bfv-\bfv^*(\varepsilon)\|_1\le C(K,A_{\mP})\varepsilon$. The upper bound on $\rmf^*$ in terms of $\bfv^*(\varepsilon)$ follows from
  \begin{align*}
  \rmf^*&\le  \langle\bff,\bfv\rangle \\
        &=    \langle\bff,\bfv - \bfv^*(\varepsilon)\rangle + \langle\bff,\bfv^*(\varepsilon)\rangle\\
        &\le  \Vert\bff\Vert_{\infty}\Vert\bfv^* - \bfv^*(\varepsilon)\Vert_{1} + \langle\bff,\bfv^*(\varepsilon)\rangle\\
        &=    \Vert\bff\Vert_{\infty}C(K,A_{\mP})\varepsilon + \langle\bff,\bfv^*(\varepsilon)\rangle.\tag*{\qed}
  \end{align*}   
\end{proof}
If the separation problem for some patterns $P$ is too hard, it might be useful to replace the corresponding moment bodies $\mM(K)_{P}$ by convex and compact approximations $M^{P}_{\varepsilon'}$, $\varepsilon'>0,$ that satisfy
\[
\mM(K)_{P}\subseteq M^{P}_{\varepsilon'}\subseteq\Neps[\varepsilon'](\mM(K)_{P}).
\] 
Since the linear constraints $\xmin{\alpha}{K}\le\rmv_\alpha\le\xmax{\alpha}{K}$ with $\alpha\in P$ are valid for $\mM(K)_P$,  one can always add these constraints to the underlying approximate description of $\mM(K)_P$. We can therefore assume that $M^{P}_{\varepsilon'}$ is a subset of $\Box(\xmin{P}{K},\xmax{P}{K})$.  Replacing the separation problems in step (2) of \cref{algo:cutting} by the separation problems 
for $M^{P}_{\varepsilon'}$ yields an algorithm that solves  
\begin{align}\tag{P'-RLX}\label{eps-RLX}  
  \begin{array}{cl@{\,}l@{\,}lll}
     \minimize{0}  & \langle\, & \multicolumn{2}{@{}l}{\bff,\bfv \, \rangle}  \\
     \for[0]{0}    &          & \bfv      & \in\R^{A_{\mP}}\\
     \st[0]{0}     &          & \bfv_{P}  & \in M^{P}_{\varepsilon'} \,\fa[0]{0}\, P\in\mP.
  \end{array}
\end{align}
This algorithm terminates after finitely many iterations. To see this, it suffices to observe that \cref{05-prop:qualitive-convergence} holds for $M^{P}_{\varepsilon'}$ in place of $\mM(K)_{P}$, since the proof of \cref{05-prop:qualitive-convergence} only relies on the convexity and compactness of $\mM(K)_{P}$. Similarly, the proof of  \cref{05-prop:quantitative-convergence} can be used without any changes to show that the optimal value  $f^{\varepsilon'}$ of \eqref{eps-RLX} and the output $\bfv^{\varepsilon'}(\varepsilon)$ of the algorithm satisfy
\begin{align}\label{05-ineq:epsRLX1}
  \langle\bff,\bfv^{\varepsilon'}(\varepsilon)\rangle \le f^{\varepsilon'}\le \Vert\bff\Vert_{\infty}C(K,A_{\mP})\varepsilon + \langle\bff,\bfv^{\varepsilon'}(\varepsilon)\rangle.
\end{align}
Since every feasible point of \eqref{eps-RLX} is $C(K,A_{\mP})\varepsilon$-feasible for \eqref{P-RLX}, we have
\begin{align}\label{05-ineq:epsRLX2}
  \rmf^*\le \|\bff\|_{\infty}C(K,A_{\mP})\varepsilon' + f^{\varepsilon'}.
\end{align}
Combining \eqref{05-ineq:epsRLX1} and \eqref{05-ineq:epsRLX2} using the triangle inequality yields  
\[
  \langle\bff,\bfv^{\varepsilon'}(\varepsilon)\rangle \le f^{*}\le \Vert\bff\Vert_{\infty}C(K,A_{\mP})(\varepsilon+\varepsilon') + \langle\bff,\bfv^{\varepsilon'}(\varepsilon)\rangle.
\]
This line of thought justifies replacing separation problems for chains and shifted chains in step (2) of \cref{algo:cutting} by their linear relaxation obtained by applying \cref{03-prop:phi} to the respective separation problem. % \eqref{03-op:sp-c-disc} and \eqref{03-op:sp-sc-disc}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Pattern Generation Routine} \label{05-subsec:pattern-generation}
%
%To be able to use Cutting Plane Algorithm \ref{cutting:plane:algorithm}, we need to develop a way of generating a family of patterns for a given nonempty set $A \subseteq \Nn$. The following is an algorithm for the generation of a family of patterns $\mathcal{P}$ for $A$ and some given pattern types $\mathrm{Type}_1,$ $\dots,$ $\mathrm{Type}_k$. To use this algorithm, we need to supply each pattern type $\mathrm{Type}_i$ with a method, which we call Find Pattern Routine, that takes a set $A_{\mP} \subseteq \Nn$ as an input and generates a family of patterns of $\mathrm{Type}_i$ connecting the elements of $A_{\mP}$. In what follows we make suggestions for Find Pattern Routine methods for the pattern types that we described in \cref{03-pat}. 
%\begin{mdframed}
%	\hs{-2pt}\textbf{Input:}  $A\subseteq\Nn$ and pattern types $\mathrm{Type}_1,$ $\dots,$ $\mathrm{Type}_k$.
%	
%	\hs{-17pt}\textbf{Output:} a family $\mathcal{P}$ of patterns of typs $\mathrm{Type}_1,$ $\dots,$ $\mathrm{Type}_k$ and a set $A_{\mP}\subseteq\Nn$ with $A\subseteqA_{\mP}$ and $A_{\mP}=\bigcup_{P\in\mathcal{P}}P$. 
%	\begin{itemize}
%		\item[(1)] 
%		Initialize 
%		\begin{itemize}
%			\item[] $A_{\mP}\leftarrow A$
%			\item[] $\mathcal{P}\leftarrow\emptyset$.
%		\end{itemize}
%		\item[(2)]
%		For all $i\in [k]$
%		\begin{itemize}
%			\item[]
%			employ Find Pattern Routine for  $\mathrm{Type}_i$ and obtain family of patterns $\mathcal{P}_i$ of $\mathrm{Type}_i$ and updated $A_{\mP}$.
%		\end{itemize}
%		\item[(3)]
%		Return the family of patterns $\mathcal{P}=\bigcup_{i\in [k]}\mathcal{P}_i$ and $A_{\mP}$.
%	\end{itemize}
%\end{mdframed}
%\begin{figure}[!h]
%	\centering
%	\includegraphics{figures/05-fig-search-order0.pdf}
%	%  \tikzsetfigurename{figures/05-fig-search-order}
%	%  \input{0figures/5-fig-search-order.tex}
%	\caption{For the given set $A$ the Pattern Generation Routine \ref{05-subsec:pattern-generation} produces different results for two different orderings of the pattern types ML and CH.}\label{05-fig-search-order}
%\end{figure}
%The output of the Pattern Generation Routine \ref{05-subsec:pattern-generation} depends on the order of the pattern types $\mathrm{Type}_1,\dots,\mathrm{Type}_k$, see \cref{05-fig-search-order}. This is because the set $A_{\mP}$ grows due to its update in the Add Pattern Routine. For dense polynomials of degree $d$, which correspond to $A=\N^n_d$, the order of the pattern types does not matter.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Add Pattern Routine} \label{05-subsec-add-pattern-routine}
%This routine adds a pattern $P$ to a given family $\mathcal{P}$ if $P$ is not already contained in a pattern of $\mathcal{P}$. 
%\begin{mdframed}
%\hs{-2pt}\textbf{Input:}  $A_{\mP}\subseteq\Nn$, a family of patterns $\mathcal{P}$ and a pattern $P$. 
%
%\hs{-17pt}\textbf{Output:} Updated $\mathcal{P}$ and $A_{\mP}$. 
%\begin{itemize}
%   \item[] If $P\not\subseteq\tilde{P}$ for all $\tilde{P}\in\mathcal{P}$
%  \begin{itemize}
%    \item[] $\mathcal{P}\leftarrow\mathcal{P}\cup\{P\}$ 
%    \item[] $A_{\mP}\leftarrowA_{\mP}\cup P$.
%  \end{itemize}
%\end{itemize}
%\end{mdframed}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Find Multilinear Pattern Routine}\label{05-subsec:find-multilinear}
%
%\begin{mdframed}
%\hs{-2pt}\textbf{Input:}  $A_{\mP}\subseteq\Nn$. 
%
%\hs{-17pt}\textbf{Output:} a family $\mathcal{P}$ of multilinear patterns and a set $A_{\mP}\subseteq\Nn$ with $A\subseteqA_{\mP}$ and $A_{\mP}=\bigcup_{P\in\mathcal{P}}P$. 
%\begin{itemize}
%  \item[(1)]
%  Initialize 
%  \begin{itemize}
%    \item[] $\mathcal{P}\leftarrow\emptyset$.
%  \end{itemize}
%  \item[(2)]
%  For $\alpha\inA_{\mP}$
%  \begin{itemize}
%    \item[]
%    use Add Pattern Routine \ref{05-subsec-add-pattern-routine} for $\ML(\alpha)$ to update $\mathcal{P}$ and $A_{\mP}$. 
%  \end{itemize}
%%  \item[(2)]
%%	For $i$ from $0$ to $n-1$ 
%%	\begin{itemize}
%%	   \item[] for all $\alpha\inA_{\mP}$ with $\|\supp(\alpha)\|=n-i$ 
%%	   \begin{itemize}
%%	     \item[]
%%	     use Add Pattern Routine \ref{05-subsec-add-pattern-routine} for $ML(\alpha)$ to update $\mathcal{P}$ and $A_{\mP}$. 
%%	    \end{itemize}
%%	\end{itemize}
%	\item[(3)]
%	Return the family of patterns $\mathcal{P}$ and $A_{\mP}$.
%\end{itemize}
%\end{mdframed}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Find Chain Pattern Routine}
%As usual, $\gcd(\alpha)$ is the greatest common divisor of the components of $\alpha \in \Nn$. For $X \subseteq \N$, $\gcd(X)$ denotes the greatest common divisor of the elements of $X$. 
%
%\begin{mdframed}
%\hs{-2pt}\textbf{Input:}  $A_{\mP}\subseteq\Nn$. 
%
%\hs{-17pt}\textbf{Output:} a family $\mathcal{P}$ of chain patterns and a set $A_{\mP}\subseteq\Nn$ with $A\subseteqA_{\mP}$ and $A_{\mP}=\bigcup_{P\in\mathcal{P}}P$. 
%\begin{itemize}
%	\item[(1)] 
%	Initialize 
%	 \begin{itemize}
%	   \item[] $\mathcal{P}\leftarrow\emptyset$.
%	 \end{itemize}
%	\item[(2)]
%	For all $\beta\in\{\frac{\alpha}{\gcd(\alpha)} :\alpha\inA_{\mP}A_{\mP}ckslash\{\0\}\}$,
%	\begin{itemize}
%	   \item[(2.1)] 
%	   let $s$ be the maximal integer value such that $s\beta\inA_{\mP}$ and 
%	   \item[] 
%	   $g=\gcd(\{t\in\N :  t\beta\inA_{\mP}\})$,
%	   \item[(2.2)]
%        then use the Add Pattern Routine \ref{05-subsec-add-pattern-routine} for $$\CH(g\beta,\tfrac{s}{g})=\llb ig\beta: i= 0,\dots,\tfrac{s}{g}\rrb$$ to update $\mathcal{P}$ and $A_{\mP}$.
%	\end{itemize}
%	\item[(3)]
%	Return the family of patterns $\mathcal{P}$ and $A_{\mP}$.
%\end{itemize}
%\end{mdframed}
%In step (2.2), we could also add the chain $\CH(\beta,s)$ instead of $\CH(g\beta,\tfrac{s}{g})$, since $\CH(g\beta,\tfrac{s}{g})\subseteq\CH(\beta,s)$. 
%	When $\CH(g \beta, \frac{s}{g})$ is generated in step (2.2), it connects the same moment variables in $A_{\mP}$ as the chain $\CH(\beta,s)$. In our algorithm, we prefer to use $\CH(g\beta, \frac{s}{g})$, because in general this chain has a smaller cardinality and therefore it introduces fewer new moment variables.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Find Shifted Chain Pattern Routine} \label{05-subsec:find-shifted-chains}
%This routine finds shifted chains with generators $\gamma=\bfe^i, i\in [n].$ We define the projection $\pi^{i}(\alpha):=(\alpha_1,\dots, \alpha_{i-1},\alpha_{i+1},\dots,\alpha_n)$ of a vector $\alpha\in\Nn$. %For a given set nonempty and finite set $A_{\mP}\subseteq\Nn$ the family $\mathcal{P}$ of chain patterns is generated in the following way. 
%\begin{mdframed}
%\hs{-2pt}\textbf{Input:}  $A_{\mP}\subseteq\Nn$. 
%
%\hs{-17pt}\textbf{Output:} a family $\mathcal{P}$ of shifted chain patterns with generators $\gamma=\bfe^i, i\in [n]$ and a set $A_{\mP}\subseteq\Nn$ with $A\subseteqA_{\mP}$ and $A_{\mP}=\bigcup_{P\in\mathcal{P}}P$,
%\begin{itemize}
%	\item[(1)] 
%	Initialize 
%	 \begin{itemize}
%	   \item[] $\mathcal{P}\leftarrow\emptyset$.
%	 \end{itemize}
%	\item[(2)]
%	For all $i\in [n]$
%      \begin{itemize}
%        \item[]
%        for all $\beta\in\pi^{i}(A_{\mP})$ 
%        \begin{itemize}
%          \item[(2.1)]
%          let $s=\max\{\alpha_i:\alpha\inA_{\mP},\,\pi^{i}(\alpha)=\beta\}$,
%          \item[]
%          $g=\gcd(\{\alpha_i: \alpha\inA_{\mP},\,\pi^{i}(\alpha)=\beta\})$ and 
%          \item[]
%          $\tilde{\alpha}=(\alpha_1,\dots, \alpha_{i-1},0,\alpha_{i+1},\dots,\alpha_n).$
%          \item[(2.2)]
%          Then use the Add Pattern Routine \ref{05-subsec-add-pattern-routine} for $$\tilde{\alpha}+\CH(g\bfe^i,\tfrac{s}{g})=\{(\alpha_1,\dots, \alpha_{i-1},jg,\alpha_{i+1},\dots,\alpha_n) : j= 0,\dots,\tfrac{s}{g}\}$$ to update $\mathcal{P}$ and $A_{\mP}$.
%        \end{itemize}
%      \end{itemize}
%	\item[(3)]
%	Return the family of patterns $\mathcal{P}$ and $A_{\mP}$.
%\end{itemize}
%\end{mdframed}
%Observe that the output depends on the order of the enumeration of $[n]$ in step (2). Consider for example $A_{\mP} = \{ (1,1), (1,3), (2,2) (4,2)\}$. Analogously to the discussion after the Find Chain Pattern Routine, in step (2.2) there is a choice between the larger chain  $\tilde{\alpha}+\CH(\bfe^i,s)$ and the chain $\tilde{\alpha}+\CH(g\bfe^i,\tfrac{s}{g})$. As before, we prefer to use smaller chains.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Find Axis Chain Pattern Routine}\label{05-subsec:find-axis-chains}
% In order to find axis chains we modify the Find Shifted Chain Pattern Routine \ref{05-subsec:find-shifted-chains} by changing step (2) as follows: let $\beta = \0$ and, for all $i \in [n]$, which satisfy $\supp (\alpha) = \{i\}$ for at least one $\alpha \in A_{\mP}$, execute steps (2.1) and (2.2).


